On the Security Risks of Knowledge Graph Reasoning

Knowledge graph reasoning (KGR) -- answering complex logical queries over large knowledge graphs -- represents an important artificial intelligence task, entailing a range of applications (e.g., cyber threat hunting). However, despite its surging popularity, the potential security risks of KGR are largely unexplored, which is concerning, given the increasing use of such capability in security-critical domains. This work represents a solid initial step towards bridging the striking gap. We systematize the security threats to KGR according to the adversary's objectives, knowledge, and attack vectors. Further, we present ROAR, a new class of attacks that instantiate a variety of such threats. Through empirical evaluation in representative use cases (e.g., medical decision support, cyber threat hunting, and commonsense reasoning), we demonstrate that ROAR is highly effective to mislead KGR to suggest pre-defined answers for target queries, yet with negligible impact on non-target ones. Finally, we explore potential countermeasures against ROAR, including filtering of potentially poisoning knowledge and training with adversarially augmented queries, which leads to several promising research directions.

==> ack.tex <==
\section*{Acknowledgement}

We thank the anonymous shepherd and reviewers for their valuable feedback. This work is supported by the National Science Foundation under Grant No. 2212323, 2119331, 1951729, and 1953893. 
Shouling Ji is partially supported by NSFC under No. 62102360.
Xiapu Luo is partially supported by HKPolyU Grant (No. ZVG0). Xusheng Xiao is partially supported by the National Science Foundation under Grant No. 2028748. 

==> benchmark.tex <==
\section{Experimental Setup}

\subsection{Reasoning cases}

We consider two reasoning scenarios as our evaluation cases: cyber threat intelligence and drug repurposing.

% \vspace{2pt}
% \noindent
% {\bf Cyber threat intelligence.} Modern cyber threats progress their attack strategies with each passing day, thus raising requirements to rely on a search engine to aid the security analyst\mcite{mittal2016cybertwitter, mittal2019cyber}. In this scenario, we build a {\it threat engine} to automatically identifies cyber threats with input evidence. The backend of a threat engine is a \kg that works as an external database and includes adversarial techniques, malware families, campaigns, etc. When a security analyst needs aid from this threat engine, the analyst extracts evidence from practical issues then constructs queries as inputs. The threat engine leverages reasoning techniques with \kg to detect threats and inspect potential solutions.

% More specifically, we build two applications in this case: 

% (1) {\bf Query threat codes --} given a set of collected evidence (\meg, affected products/versions, TTPs, or campaigns) from cybersecurity issues, the threat engine aims to find what are threat codes (\meg, CVE codes\footnote{https://cve.mitre.org}) involved in those issues; 

% (2) {\bf Query mitigation --} this is a step further than querying threat codes. The threat engine recommends potential mitigation approaches (\meg, patches, workarounds, etc.) to solve security issues.

% Moreover, we also consider a zero-day scenario in \msec{ssec:zeroday}, where the query evidence corresponds to novel threat codes not collected by \kg. The cyber engine infers mitigation approaches that potentially applicable to those zero-day threats.

\vspace{2pt}
\noindent
{\bf Drug repurposing.} Drug repurposing aims to find potential functionalities of new drugs, hence fully exploiting their therapeutic values or unknown side effects\mcite{pushpakom2019drug, oprea2011drug}. With the auxiliary of reasoning techniques, researchers can more efficiently explore interactions between drugs and their targets, such as diseases or genes. Even though the reasoning results still need to be verified by biomedical tests, the reasoning-based approaches significantly save efforts from enumerating all repurposing candidates.

Here we consider two applications to address the drug repurposing task: 

(1) {\bf Drug-disease interactions --} given a pair of drug-disease terms with their relevant properties, we aim to explore how the drug interacts with this disease.

(2) {\bf Drug-gene interactions --} given a pair of drug-gene terms with their relevant properties, we aim to find how does the gene influence the functionality of this drug.

In summary, we use the ontological reasoning mechanism in cyber threat intelligence and aim to find the threat codes and mitigation entities with given evidence. We treat the drug repurposing task as a relational reasoning problem, where we focus on inferring correct interactions between drugs and their targets despite other biomedical use cases\mcite{zhu2020knowledge, zhang2021drug}.


% \vspace{4pt}
% \begin{table*}[!ht]
% \setlength\extrarowheight{1pt}
% \centering
% \setlength{\tabcolsep}{3pt}
% {\footnotesize
% \begin{tabular}{ ccclr|lr|lrcclr|lr|lrcclr|lr|lr}
%  \toprule
%  \multirow{2}{*}{Applications} & & & \multicolumn{22}{c}{ Reasoning Results with Different Query Structures (MRR $\vert$ NDCG@5)} \\ 
% %  \cline{4-25} 
%  \cmidrule(){4-25}
%   & & &
%   \multicolumn{2}{c}{3-I} & \multicolumn{2}{c}{3-II} & \multicolumn{2}{c}{3-III} & 
%   & &
%   \multicolumn{2}{c}{5-I} & \multicolumn{2}{c}{5-II} & \multicolumn{2}{c}{5-III} &
%   & &
%   \multicolumn{2}{c}{7-I} & \multicolumn{2}{c}{7-II} & \multicolumn{2}{c}{7-III} \\
%   \midrule
% \multicolumn{1}{l}{\ding{182} Threat Code} & & & 0.63 & 0.82 & 0.56 & 0.75 & 0.56 & 0.73 & & & 0.64 & 0.79 & 0.60 & 0.75 & 0.58 & 0.74 & & & 0.64 & 0.77 & 0.63 & 0.75 & 0.63 & 0.73 \\
% %  \cline{1-19}
%  \multicolumn{1}{l}{\ding{183} Mitigation} & & & 0.50 & 0.74 & 0.43 & 0.65 & 0.42 & 0.65 & & & 0.51 & 0.70 & 0.47 & 0.65 & 0.45 & 0.64 & & & 0.51 & 0.69 & 0.47 & 0.62 & 0.49 & 0.64 \\
%  \bottomrule
%  \end{tabular}
% \caption{\footnotesize Reasoning performances on our case study I -- cyber threat intelligence. Query structures are named as {\it path num}--{\it complexity level}, see Figure \mref{fig:query:struc}. \label{tab:case1:benign}}}
% \end{table*}


% \subsection{Attacks}
% To our best knowledge, this work is the first to discuss practical security issues on reasoning systems. We thus compare attacks with different capabilities of attack vectors:
% \begin{mitemize}
% \setlength\itemsep{0.5pt}
% \item $\vect{SA}_{\vect{kgp}}$ -- The \underline{s}tand\underline{a}lone \kgp attack. The attacker is only accessible to \kg as a malicious contributor. A poisoned \kg affects downstream embedding and reasoning without further manipulation of the \kgp attacker.
% \item $\vect{SA}_{\vect{lqe}}$ -- The \underline{s}tand\underline{a}lone \lqe attack. The attacker locates at downstream use cases, thus only affects query contents, including anchor entities and logical structures.
% \item $\vect{CoP}$ -- The \underline{c}o-\underline{o}ptimization attack between \kgp and \lqe, where the downstream \lqe attacker returns specific anchor entities to \kgp attacker for stronger poisoning. Both \kgp and \lqe co-optimize their attacks on a substitute system.
% \end{mitemize}

% We also evaluate on $\ssub{Q}{tar}$ without any attacks as one baseline comparison, to see what are the performance variations with/without attacks.

%\subsection{Evaluation Metrics}

% We use three metrics to evaluate reasoning performances and attacks:
% ({\em i}) \textbf{\textit{MRR}} evaluates the mean reciprocal ranks of all answers among all queries. This metric concerns a global rank quality of reasoning answers. 
% ({\em ii}) \textbf{\textit{HIT@K}} evaluates whether top-$K$ results contain ground-truth answers. For each query, this metric gives a binary indication (0/1). We average those binary results and get a global hits ratio.
% ({\em iii}) \textbf{\textit{NDCG@K}} evaluates the ranking quality of top-$K$ results with the NDCG metric\mcite{}\ting{cite sth}, which is more strict than {\it HIT@K} since positions of ground-truth answers in top-$K$ ranks affects its value.

% The definition is:
% \begin{equation}
% \begin{split}
% \begin{gathered}
%     \text{MRR} = \frac{1}{|Q|} \sum_{q \in Q}^{} \frac{1}{|A|} \sum_{j=1}^{|A|} \frac{1}{rank\left(A\left[j\right]\right)}
% \end{gathered}
% \end{split}
% \label{eq:mrr}
% \end{equation}

% \noindent
% each query $q \in Q$ has an answer set $A$. Thus we first calculate the mean reciprocal rank of each answer for each $q$, then get the query-level mean value.



%\vspace{2pt}
\begin{table}[!ht]
\setlength\extrarowheight{1pt}
\centering
\setlength{\tabcolsep}{2pt}
{\footnotesize
\begin{tabular}{ lclclclclcr}
%  \toprule
% \Xhline{1.5\arrayrulewidth}
 Setting & & Studied cases & & Applications & & Model & & \multicolumn{3}{l}{Results} \\ 
    % \hline
    \cmidrule(){1-11}
    ontological & & I. cyber threat & & \ding{182} Threat Code & & \multirow{2}{*}{Query2Box} & & 0.61 & &  0.76 \\ 
    reasoning & & intelligence & & \ding{183} Mitigation & & &  & 0.47 & &  0.66 \\
    % \hline
    \cmidrule(){1-11}
    relational & & II. drug & & \ding{182} Drug-Disease & & GQE & & \multicolumn{3}{c}{0.73} \\ 
    reasoning & & repurposing & & \ding{183} Drug-Gene & & + R-GCN & & \multicolumn{3}{c}{0.77} \\
    %  \bottomrule
 \end{tabular}
\caption{\footnotesize Two studied reasoning scenarios and their performances. For cyber intelligence, results are MRR (left) and NDCG@5 (right); for drug repurposing, results are HIT@1. \label{tab:benign:all}}}
\end{table}

%\vspace{2pt}


==> case1.tex <==
\section{Case Study I: Cyber-Threat Hunting}
\label{sec:cyber:case}

Next, we conduct an empirical evaluation of \system in the concrete case of cyber-threat intelligence reasoning. Our study is designed to answer the following questions: Q$_1$ -- Is \system effective against \krl systems in practice?
Q$_2$ -- How does the effectiveness of its variants differ? Q$_3$ -- What factors impact the performance of \system?

\subsection{Experimental setup}

We begin by describing the evaluation setting.

\vspace{2pt}
{\bf Scenario --} With the explosive growth of cyber-threat intelligence, it becomes imperative for security analysts to rely on automated tools to extract useful, actionable intelligence for given incidents\mcite{mittal2016cybertwitter, mittal2019cyber}. Here, we consider a \krl system built upon cyber-threat KGs (\meg, attack tactics, vulnerabilities, fixes), which supports the following queries: 

\vspace{1pt}
{\em Vulnerability --} Given certain observations regarding the incident (\meg, affected products/versions, attack tactics, or campaigns), it finds the most likely vulnerabilities (\meg, \cves) that are being exploited.

\vspace{1pt}
{\em Mitigation --} Beyond the vulnerabilities being attacks, it may further suggest potential solutions (\meg, patches and workarounds) to mitigate such vulnerabilities. 

\vspace{1pt}
Besides querying for known vulnerabilities, we also consider a zero-day setting wherein the attacks exploit previously unknown vulnerabilities. 


\vspace{2pt}
{\bf CyberKG --} We construct the CyberKG using cyber-threat intelligence from three sources: ({\em i}) public \cve reports\footnote{https://www.cvedetails.com}; ({\em ii}) BRON threat graph\mcite{bron}; ({\em iii}) National Vulnerability Database ({\small NVD})\footnote{https://nvd.nist.gov}.

\vspace{1pt}
-- From ({\em i}), we collect known {\sl CVE} as potential vulnerabilities, each associated with {\sl affected product}, {\sl version}, {\sl vendor}, {\sl CWE}\footnote{https://cwe.mitre.org}, and {\sl threat campaign}. 

\vspace{1pt}
-- From ({\em ii}), we extract {\sl attack tactic}, {\sl technique} and {\sl pattern}, and link them with ({\it i}) based on \cve codes.


\vspace{1pt}
-- From ({\it iii}), we collect {\sl mitigation} for each \cve and assign a specific code to each mitigation approach. 

\vspace{1pt}
The logical structures of the resulted \kg is illustrated in Figure\mref{fig:cyberkg}, with its statistics summarized in Table\mref{tab:cyber:stat}.

\vspace{2pt}
{\bf Query -- } To construct queries, for given {\sl CVE} or {\sl mitigation}, we randomly select 
anchors from the remaining entities (\meg, {\sl affected product}, {\sl attack pattern}, and {\sl threat campaign}) and formulate the queries based on their logical structures in the KG. 
Figure\mref{fig:cyber:qpath} shows the logical paths with different anchor entities, which are combined to formulate the query templates as shown in Figure\mref{fig:cyber:qstruc}. In the evaluation,  we generate 500 queries for each query template. 

\vspace{2pt}
{\bf KRL --} We apply Query2Box\mcite{query2box}, a state-of-the-art \krl approach, to build the reasoning system. Intuitively, by adopting box embeddings (\mie, hyper-rectangles), Query2Box naturally handles first-order conjunctive queries. 


%\vspace{2pt}
\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
%\setlength{\tabcolsep}{2pt}
{\small
 \begin{tabular}{c|cc}
%  \toprule
% \Xhline{1.5\arrayrulewidth}
 Query &  MRR & NDCG@5 \\ 
\hline 
\hline
Vulnerability & 0.61 &  0.76 \\ 
Mitigation & 0.47 &   0.66 \\
 \end{tabular}
 
\caption{\krl performance in cyber-threat hunting. \label{tab:benign:all}}}
\end{table}


\vspace{2pt}
{\bf Metrics --} In this case study, we mainly use two metrics to evaluate the performance of \krl and attacks:

{\mrr} -- It computes the average reciprocal ranks of all the ground-truth answers across all the queries. This metric measures the global ranking quality of reasoning answers. 

{\ndcg} -- It evaluates the ranking quality of the top-$K$ answers using the NDCG metric\mcite{metrics}.

All the measurements range from 0 to 1, with larger values indicating better performance. Table\mref{tab:benign:all} summarizes the performance of the \krl system in cyber-threat hunting.


\subsection{Attack implementation}

\label{sec:case1:attack}

Next, we detail the implementation of \system attacks in the case study of cyber-threat hunting.

\vspace{2pt}
{\bf Attack settings --} By default, we set target queries $\gQ^*$ as that containing a specific pattern $p^* = \textsf{\small Android OS} \xrightarrow[]{\text{vulnerable to}} v_\text{CVE} \xrightarrow[]{\text{fixable by}} v_\text{mitigation}$, where 
$\textsf{\small Android OS}$ is an anchor entity while both $v_\text{CVE}$ and $v_\text{mitigation}$ are variables. In \msec{sec:case1:eval}, we also consider alternative definitions of $p^*$.

We consider both targeted and untargeted attacks. In untargeted attacks, the goal is to direct the answering of each query $q \in \gQ^*$ to an erroneous one (different from its ground-truth $\llbracket q \rrbracket$); in targeted attacks, the goal is to direct the answering of all the queries in $\gQ^*$ to a target answer $A$. For vulnerability queries, we set $A = \textsf{\small \cve-2021-0471}$, which is a \cve with lower severity among all the Android \cves; for mitigation queries, we set $A$ as the mitigation of $\textsf{\small CVE-2021-0471}$.

Further, it is necessary to ensure the impact of the attacks on benign queries (\mie, without $p^*$) is limited.


{\bf Attack variants --} To the best of our knowledge, this is the first work on the security of \krl. We thus mainly compare the performance of different variants of \system:

\vspace{1pt}
\akp -- Relying on knowledge poisoning, the adversary influences \krl by committing poisoning facts to the \kg construction, but has no control over the queries. Specifically, \akp commits poisoning facts surrounding $\textsf{\small Android OS}$ (anchor entity of $p^*$) and $\textsf{\small CVE-2021-0471}$ (target answer $A$). We limit the number of poisoning facts by $n_\mathrm{kp} = 100$.


\vspace{1pt}
\aqp -- Relying on query perturbation, the adversary generates adversarial queries at inference time but has no control over the \kg construction. To make the perturbation evasive, we require that \mcounter{i} the number of logical paths in the perturbation is limited by  $n_\mathrm{qp} = 2$ and \mcounter{ii} the dependency graph of the perturbed query is valid with respect to the \kg. 

\vspace{1pt}
\aco  -- Leveraging both knowledge poisoning and query perturbation, the adversary optimizes the poisoning facts and adversarial queries jointly. 

\vspace{1pt}
In all the attacks, we assume the adversary has no control over the training of \krl including \mcounter{i} how the training set is sampled from the \kg and \mcounter{ii} how the entity embedding and relation transformation models are trained. Thus, all the poisoning facts and/or adversarial queries are crafted on surrogate models.

\subsection{Evaluation results}
\label{sec:case1:eval}

For exposition simplicity, below we highlight the \krl performance variation before and after the attacks. In targeted attacks, ``$\uparrow$'' indicates the score increase (\meg, \mrr) with respect to target answer $A$; in untargeted attacks, ``$\downarrow$'' indicates the score decrease with respect to ground-truth answers.

\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{2pt}
{\footnotesize
\begin{tabular}{ c|c|lr|lr|lr|lr}
 \multirow{2}{*}{Objetive} & \multirow{2}{*}{Query} & \multicolumn{8}{c}{Attack} \\ 
 \cline{3-10} 
  & & \multicolumn{2}{c|}{w/o} &\multicolumn{2}{c|}{\akp} & \multicolumn{2}{c|}{\aqp} & \multicolumn{2}{c}{\aco} \\
  \hline
  \hline
 \multirow{2}{*}{Targeted} & Vulnerability & .00 & .00 & .53$\uparrow$ & .57$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .99$\uparrow$ & .99$\uparrow$ \\
   &  Mitigation & .00 & .00 & .29$\uparrow$ & .33$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .58$\uparrow$ & .60$\uparrow$ \\
  \hline
 \multirow{2}{*}{Untargeted} & Vulnerability & .56 & .75 & .34$\downarrow$ & .22$\downarrow$ & .49$\downarrow$ & .48$\downarrow$ & .55$\downarrow$ & .73$\downarrow$\\
  &  Mitigation & .48 & .68 & .31$\downarrow$ & .20$\downarrow$ & .45$\downarrow$ & .57$\downarrow$ & .48$\downarrow$ & .68$\downarrow$ \\
 \hline
 \end{tabular}
\caption{Overall attack performance in cyber-threat hunting. Note: the values in each cell are MRR (left) and NDCG@5 (right).\label{tab:cyber:attack:overall}}}
\end{table}

\vspace{2pt}
{\bf Attack effectiveness --} Table\mref{tab:cyber:attack:overall} summarizes the overall attack performance measured by \mrr and \ndcgf. Note that without attacks (w/o), none of the queries in $\gQ^*$ leads to target answer $A$, due to their irrelevance. We have the following interesting observations.

\underline{\textit{\akp is more effective in targeted attacks.}} -- \aqp seems unable to direct \krl to target answer $A$. This may be explained by that limited by the perturbation constraints (\msec{sec:qp}), it is difficult to direct the answering of query $q$ to $A$ remotely relevant to $\llbracket q \rrbracket$. In contrast, \akp exerts a more significant influence on \krl by minimizing the distance between the embeddings of pattern $p^*$ (shared by $\gQ^*$) and $A$, leading to more effective targeted attacks.

\underline{\textit{\aqp is more effective in untargeted attacks.}} -- Interestingly, \aqp outperforms \akp in untargeted attacks. This may be explained as follows. An untargeted attack succeeds if the answer of query $q$ deviates from $\llbracket q \rrbracket$; the poisoning facts of \akp affects all the queries in the same manner, while in \aqp, the perturbation is tailored to each query $q$, resulting in more effective untargeted attacks.

\underline{\textit{\aco is the most effective attack.}} -- In both targeted and untargeted cases, \aco outperforms the other attacks. For instance, in targeted attacks against vulnerability queries, \aco attains 0.99 increase in \mrr. This may be attributed to the mutual reinforcement between knowledge poisoning and query perturbation: tailoring poisoning facts to adversarial queries, and vice versa, improves the attack effectiveness. 


\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{4pt}
{\footnotesize
\begin{tabular}{c|c|lr|lr}
 \multirow{2}{*}{Objective} & \multirow{2}{*}{Query} & \multicolumn{4}{c}{Attack} \\ 
 \cline{3-6} 
%  \cmidrule(lr){5-8}
  & & \multicolumn{2}{c|}{\akp} & \multicolumn{2}{c}{\aco} \\
  \hline
  \hline
  \multirow{2}{*}{Targeted} & Vulnerability & 0.00$\downarrow$  & 0.00$\downarrow$ & 0.00$\downarrow$ & 0.00$\downarrow$ \\
   & Mitigation & 0.01$\downarrow$ & 0.00$\downarrow$ & 0.00$\downarrow$ & 0.02$\downarrow$ \\
  \hline
 \multirow{2}{*}{Untargeted} & Vulnerability & 0.00$\downarrow$ & 0.02$\downarrow$ & 0.00$\downarrow$  &  0.00$\downarrow$ \\
 & Mitigation  & 0.01$\downarrow$  & 0.01$\downarrow$ & 0.00$\downarrow$ & 0.00$\downarrow$ \\
 \hline
 \end{tabular}
\caption{\small Impact of attacks on non-target queries. Note: the values in each cell are MRR (left) and NDCG@5 (right). \label{tab:benign:drop:cyber}}}
\end{table}

\vspace{2pt}
{\bf Attack evasiveness --} We further measure the impact of the attacks on non-target queries (without pattern $p^*$). As \aqp has no influence on non-target queries, we focus on evaluating \akp and \aco, with results shown in  Table\mref{tab:benign:drop:cyber}. 

\underline{{\em \system has a limited impact on non-target queries.}} -- Compared with the benign system ({\em cf.} Table\mref{tab:benign:all}), \akp and \aco have negligible influence on the answering of non-target queries. This may be attributed to multiple factors: \mcounter{i} the limited number of poisoning facts (less than $n_\mathrm{kp}$), \mcounter{ii} the locality of such facts, and 
\mcounter{iii} the large size of \kg.

\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{2pt}
{\footnotesize
\begin{tabular}{ cccccc|cc|cccccc|cc|cccccc|cc|cc}
%  \toprule
\hline
 \multirow{2}{*}{Objective} &  \multirow{2}{*}{Attack} & & & \multicolumn{22}{c}{ Query Topological Structure ($n_\mathrm{path}$-$m_\mathrm{path}$)} \\ 
 \cline{5-26} 
%  \cmidrule(lr){5-26}
  & & & &
  \multicolumn{2}{c}{3-1} & \multicolumn{2}{c}{3-2} & \multicolumn{2}{c}{3-3} & 
  & &
  \multicolumn{2}{c}{5-1} & \multicolumn{2}{c}{5-2} & \multicolumn{2}{c}{5-3} &
  & &
  \multicolumn{2}{c}{7-1} & \multicolumn{2}{c}{7-2} & \multicolumn{2}{c}{7-3} \\
%   \midrule
\hline
\hline
 & w/o & & & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & & & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & & & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\multirow{2}{*}{Targeted} & \akp & & & 0.51$\uparrow$ & 0.56$\uparrow$ & 0.78$\uparrow$ & 0.81$\uparrow$ & 0.78$\uparrow$ & 0.81$\uparrow$ & & & 0.37$\uparrow$ & 0.40$\uparrow$ & 0.63$\uparrow$ & 0.71$\uparrow$ & 0.66$\uparrow$ & 0.71$\uparrow$ & & & 0.23$\uparrow$ & 0.27$\uparrow$ & 0.38$\uparrow$ & 0.42$\uparrow$ & 0.39$\uparrow$ & 0.44$\uparrow$ \\
& \aqp & & & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c}{\NA} & & & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c}{\NA} & & & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c}{\NA} \\
& \aco & & & 0.98$\uparrow$ & 0.98$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & & & 0.97$\uparrow$ & 0.98$\uparrow$ & 1.00$\uparrow$ & 0.99$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & & & 0.94$\uparrow$ & 0.96$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ & 1.00$\uparrow$ \\
% \midrule
\hline
 & w/o & & & 0.59 & 0.83 & 0.52 & 0.75 & 0.52 & 0.74 & & & 0.60 & 0.78 & 0.56 & 0.75 & 0.54 & 0.72 & & & 0.60 & 0.76 & 0.56 & 0.72 & 0.58 & 0.72 \\
\multirow{2}{*}{Untargeted} & \akp & & & 0.35$\downarrow$ & 0.24$\downarrow$ & 0.31$\downarrow$ & 0.30$\downarrow$ & 0.42$\downarrow$ & 0.40$\downarrow$ & & & 0.34$\downarrow$ & 0.19$\downarrow$ & 0.34$\downarrow$ & 0.25$\downarrow$ & 0.35$\downarrow$ & 0.28$\downarrow$ & & & 0.31$\downarrow$ & 0.12$\downarrow$ & 0.33$\downarrow$ & 0.09$\downarrow$ & 0.36$\downarrow$ & 0.11$\downarrow$ \\
& \aqp & & & 0.50$\downarrow$ & 0.54$\downarrow$ & 0.51$\downarrow$ & 0.66$\downarrow$ & 0.51$\downarrow$ & 0.65$\downarrow$ & & & 0.50$\downarrow$ & 0.41$\downarrow$ & 0.49$\downarrow$ & 0.46$\downarrow$ & 0.47$\downarrow$ & 0.44$\downarrow$ & & & 0.50$\downarrow$ & 0.37$\downarrow$ & 0.47$\downarrow$ & 0.41$\downarrow$ & 0.49$\downarrow$ & 0.41$\downarrow$ \\
& \aco & & & 0.58$\downarrow$ & 0.81$\downarrow$ & 0.52$\downarrow$ & 0.75$\downarrow$ & 0.52$\downarrow$ & 0.74$\downarrow$ & & & 0.58$\downarrow$ & 0.74$\downarrow$ & 0.54$\downarrow$ & 0.73$\downarrow$ & 0.53$\downarrow$ & 0.71$\downarrow$ & & & 0.57$\downarrow$ & 0.70$\downarrow$ & 0.55$\downarrow$ & 0.71$\downarrow$ & 0.57$\downarrow$ & 0.71$\downarrow$ \\
 \hline
 \end{tabular}
\caption{\small Topological complexity of queries on the attack performance. Note: the values in each cell are MRR (left) and NDCG@5 (right). \label{tab:cyber:attack:diff:struc}}}
\end{table*}


\vspace{2pt}
\textbf{Query structures --} Recall that the queries are generated following a set of templates ({\em cf.} Figure\mref{fig:cyber:qstruc}). We now evaluate the impact of query structures on the attack performance. We encode the complexity of query $q$ as $n_\mathrm{path}$-$m_\mathrm{path}$, where 
$n_\mathrm{path}$ is the number of logical paths (from anchors $\gK_q$ to answer $\llbracket q \rrbracket$) in $q$ and $m_\mathrm{path}$ is the length of the longest path. Table\mref{tab:cyber:attack:diff:struc} breaks down the attack performance according to the setting of $n_\mathrm{path}$ and $m_\mathrm{path}$. We have the following observations.


\underline{{\em Attack performance drops with $n_\mathrm{path}$.}} -- By increasing the number of logical paths $n_\mathrm{path}$ but keeping the maximum path length $m_\mathrm{path}$ fixed, the effectiveness of all the attacks tends to drop. This may be explained as follows. Each logical path in query $q$ represents one constraint on the answer $\llbracket q \rrbracket$; with more constraints, \krl is more robust to local perturbation to either \kg or parts of $q$.

\underline{{\em Attack performance improves with $m_\mathrm{path}$ in targeted cases.}} -- Interestingly, in the targeted cases, the attack performance improves with $m_\mathrm{path}$ under fixed $n_\mathrm{path}$. This may be explained as follows. Longer logical paths in $q$ represent ``weaker'' constraints, due to the accumulated approximation errors of relation transformation. As $p^*$ is defined as a short logical path, for queries with large $m_\mathrm{path}$, $p^*$ tends to dominate the query answering, resulting in more effective attacks.


\begin{figure*}
    \centering
    \epsfig{file = figures/cyber_cop_3D_ndcg.pdf, width = 170mm}
    \caption{NDCG@5 variation of \aco as a function of knowledge poisoning budget ($n_\mathrm{kp}$) and query perturbation budget ($n_\mathrm{qp}$).}
    \label{fig:cyber:cop:ndcg}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \epsfig{file = figures/cyber_cop_3D_mrr.pdf, width = 170mm}
    \caption{MRR variation of \aco with respect to knowledge poisoning budget ($n_\mathrm{kp}$) and query perturbation budget ($n_\mathrm{qp}$).}
    \label{fig:cyber:cop:mrr}
\end{figure*}




\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{2.5pt}
{\footnotesize
\begin{tabular}{ c|c|lr|lr|lr}
 \multirow{2}{*}{Objective} & \multirow{2}{*}{Query} & \multicolumn{6}{c}{Attack} \\ 
 \cline{3-8} 
  & &\multicolumn{2}{c|}{\akp} & \multicolumn{2}{c|}{\aqp} & \multicolumn{2}{c}{\aco} \\
  \hline
  \hline
  \multicolumn{8}{c}{Embedding Dimensionality = 200, DNN Depth = 1} \\
   \hline
 \multirow{2}{*}{Targeted} & Vulnerability & .48$\uparrow$ & .55$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .96$\uparrow$ & .99$\uparrow$ \\
  & Mitigation & .26$\uparrow$ & .31$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .50$\uparrow$ & .55$\uparrow$ \\
  \hline
 \multirow{2}{*}{Untargeted} & Vulnerability &  .34$\downarrow$ & .22$\downarrow$ & .47$\downarrow$ & .44$\downarrow$ & .51$\downarrow$ & .70$\downarrow$\\
 & Mitigation & .27$\downarrow$ & .21$\downarrow$ & .40$\downarrow$ & .54$\downarrow$ & .44$\downarrow$ & .62$\downarrow$ \\
 \hline
 \multicolumn{8}{c}{Embedding Dimensionality = 500, DNN Depth = 4} \\
  \hline
  \multirow{2}{*}{Targeted} & Vulnerability & .50$\uparrow$ & .56$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .91$\uparrow$ & .95$\uparrow$ \\
 & Mitigation &  .27$\uparrow$ & .33$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .52$\uparrow$ & .54$\uparrow$ \\
  \hline
  \multirow{2}{*}{Untargeted} & Vulnerability &  .30$\downarrow$ & .19$\downarrow$ & .44$\downarrow$ & .36$\downarrow$ & .49$\downarrow$ & .63$\downarrow$\\
 & Mitigation & .22$\downarrow$ & .15$\downarrow$ & .37$\downarrow$ & .42$\downarrow$ & .40$\downarrow$ & .61$\downarrow$ \\
 \hline
 \end{tabular}
\caption{Attack performance under alternative surrogate models.\label{tab:cyber:surrogate}}}
\end{table}

\vspace{2pt}
\textbf{Surrogate models --} Thus far, we assume the surrogate models on which the adversary crafts poisoning facts and/or adversarial queries share the same architectures with the target \krl system. We now examine the scenario wherein the surrogate and actual models differ. 

We consider two configurations of the surrogate models different from the actual models used by \krl ({\em c.f.} Table\mref{tab:model}) in terms of \mcounter{i} the dimensionality of embeddings and \mcounter{ii} the depth of \dnns (as relation transformation models), while all the other settings are the same as Table\mref{tab:cyber:attack:overall}. Table\mref{tab:cyber:surrogate} shows the attack performance under such alternative surrogate models.

\underline{{\em \system transfers across different embedding models.}} -- By comparing Table\mref{tab:cyber:surrogate} and Table\mref{tab:cyber:attack:overall}, it is observed that while the attack performance drops under the alternative settings, due to the discrepancy between the actual and surrogate models, the decrease is marginal, indicating the transferability of \system across different models. This may be explained by that many \kg embedding methods demonstrate fairly similar behavior\mcite{bilinear-embedding}. It is therefore possible to transfer attacks across different embedding models.


\begin{figure*}
    \centering
    \epsfig{file = figures/cyber_diff_ltar.pdf, width = 170mm}
    \caption{Attack performance under alternative definitions of $p^*$.}
    \label{fig:cyber:diff:tar:logic}
\end{figure*}

\vspace{2pt}
\textbf{KG-Query interaction --} We further evaluate the interaction between the attack vectors of knowledge poisoning and query perturbation in \aco. Specifically, we evaluate the attack performance as a function of $n_\mathrm{kp}$ (number of injected poisoning facts) and $n_\mathrm{qp}$ (number of perturbed logical paths), with results summarized in Figure\mref{fig:cyber:cop:ndcg}.

\underline{{\em There exists an ``mutual reinforcement'' effect.}} -- In both targeted and untargeted cases, with $n_\mathrm{qp}$ fixed, slightly increasing $n_\mathrm{kp}$ significantly improves the attack performance. For instance, in targeted cases, when $n_\mathrm{kp} = 0$, \ndcgf remains 0 regardless of the setting of $n_\mathrm{kp}$; if $n_\mathrm{kp} = 50$, even setting $n_\mathrm{qp} = 1$ leads to \ndcgf over 0.5. This indicates that knowledge poisoning greatly boosts the effectiveness of query perturbation and also validates the analysis in \msec{sec:co}.

\underline{{\em The effect is even more evident in untargeted attacks.}} -- It is also observed that \system achieves its maximum effectiveness in untargeted attacks with $n_\mathrm{kp}$ and $n_\mathrm{qp}$ lower than the case of targeted attacks. This is explained by that without the need to direct \krl to a specific answer $A$, untargeted attacks are relatively ``easier'' than targeted attacks, making the mutual reinforcement even more significant.

We also observe similar trends measured by \mrr with results shown in Figure\mref{fig:cyber:cop:mrr}. % (\msec{sec:additional}).


\vspace{2pt}
\textbf{Alternative $p^*$ pattern --} The pattern $p^*$ serves a trigger to invoke \krl to malfunction in \akp and \aco. Here, we consider alternative definitions of $p^*$ and evaluate its impact on the attack performance. Specifically, besides its default definition (with $\textsf{\small Android OS}$ as anchor) in \msec{sec:case1:attack}, we consider two other definitions as listed in Table\mref{tab:diff:tar:logic}: the one has $\textsf{\small Port Scanning}$ (which refers to an {\sl attack pattern}) as its anchor and its logical path is of length 2; the other has $\textsf{\small T1033}$ (which refers to an {\sl attack technique} of ``system owner/user discovery technique''\footnote{https://attack.mitre.org/techniques/T1033/}) as its anchor and is of length 3. 

\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{2.0pt}
{\footnotesize
\begin{tabular}{ c|ccc}
Anchor of $p^*$ & $\mathsf{Android\,\,OS}$ & $\mathsf{Port\,\,Scanning}$ & $\mathsf{T1033}$\\
\hline
Category & $\mathsf{Product}$ & $\mathsf{Attack\,\,pattern}$ & $\mathsf{Technique}$ \\
Length (Vulnerability) & 1 hop & 2 hop & 3 hop \\
Length (Mitigation) & 2 hop & 3 hop & 4 hop \\
\end{tabular}
\caption{Alternative definitions of $p^*$. \label{tab:diff:tar:logic}}}
\end{table}

\underline{{\em $p^*$ with shorter paths leads to more effective attacks.}} -- In Figure\mref{fig:cyber:diff:tar:logic}, we compares the attack performance of \akp and \aco under varying definitions of $p^*$ in both targeted and untargeted cases. Observe that the attack effectiveness decreases as the length of $p^*$ grows. This can be explained as follows. As the poisoning facts are selected surrounding the anchors, their influence tends to fade as the distance between the anchors and the answers. Further, while \akp is inefficient under the setting of $p^*$ starting with $\textsf{\small T1033}$, \aco is much less sensitive to the setting of $p^*$ (\meg, \mrr $\geq 0.39$ and \ndcgf $\geq 0.42$), indicating the necessity of co-optimizing poisoning facts and adversarial queries.  


\vspace{2pt}
{\bf Zero-day threats --} We further evaluate the performance of \system in the scenario of {\it zero-day} threats, wherein the threats exploit previously unknown vulnerabilities, which often result in consequential damages in practice\mcite{zero-day}.  
We simulate the zero-day case by randomly removing 30\% \cves (from 2020 to 2021) from the \kg as the zero-day vulnerabilities, then generating queries with ground-truth answers among the deleted \cves. The reasoning task is to search for potential {\sl mitigation} for given incidents. Intuitively, it is possible to find correct mitigation even though the vulnerability is unknown based on similar vulnerabilities (\mie, approximate query). Meanwhile, the attacks aims to mislead \krl to erroneous suggestions (untargeted) or a specific {\sl mitigation} $A = \textsf{{\small MITI-72591}}$\footnote{https://source.android.com/security/bulletin/2021-04-01} (targeted).

\vspace{2pt}
\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{3pt}
{\footnotesize
\begin{tabular}{ c|lr|lr|lr|lr}

 \multirow{2}{*}{Objective} & \multicolumn{8}{c}{Attack} \\ 
 \cline{2-9} 
  & \multicolumn{2}{c|}{w/o} & \multicolumn{2}{c|}{\akp} & \multicolumn{2}{c|}{\aqp} & \multicolumn{2}{c}{\aco} \\
  \hline
  \hline
 Targeted &  .00 & .00 & .34$\uparrow$ & .40$\uparrow$ & \multicolumn{1}{c}{\NA} & \multicolumn{1}{c|}{\NA} & .47$\uparrow$ & .55$\uparrow$ \\
 Untargeted &  .39 & .61 & .20$\downarrow$ & .22$\downarrow$ & .30$\downarrow$ & .44$\downarrow$ & .39$\downarrow$ & .59$\downarrow$ \\
 \hline
 \end{tabular}
\caption{Attack performance against zero-day threat queries. \label{tab:cyber:attack:zeroday}}}
\end{table}

\underline{{\em \system is also effective against approximate queries.}} -- Table\mref{tab:cyber:attack:zeroday} presents the attack performance in zero-day case. Comparing with Table\mref{tab:cyber:attack:overall}, we have similar observations that ({\em i}) \akp is more effective than \aqp in targeted attacks; ({\em ii}) \aqp is more effective than \akp in untargeted attacks; and ({\em iii}) \aco is the most effective among the three.

Also, note that \system is marginally less effective against approximate queries, due to the missing links (\mie, {\sl Vulnerability}) on the paths from anchor entities to answers ({\sl Mitigation}). However, as similar vulnerabilities tend to share mitigation, \system is still able to craft effective poisoning facts/adversarial queries to mislead \krl.


==> case2.tex <==
\section{Case Study II: Drug Repurposing}
\label{sec:drug:case}

In the case of cyber-threat hunting, we evaluate \system over queries regarding \kg entities. Below, we further evaluate \system over queries regarding \kg relations in the concrete case of drug repurposing reasoning. 

\subsection{Experimental setup}

We begin by describing the evaluation setting.

\vspace{2pt}
{\bf Scenario --} Drug repurposing aims to find potential therapeutic values or unknown side effects of new drugs\mcite{pushpakom2019drug, oprea2011drug} by exploring the interactions between drugs, diseases, and human genes. To this end, we consider a \krl system built upon knowledge regarding drugs, diseases, and genes, which supports the following queries:

% With the auxiliary of reasoning techniques, researchers can more efficiently explore interactions between drugs and their targets, such as diseases or genes. Even though the reasoning results still need to be verified by biomedical tests, the reasoning-based approaches significantly save efforts from enumerating all repurposing candidates.

% Here we consider two applications to address the drug repurposing task: 

{\em Drug-disease interaction --} Given a drug-disease pair  with their relevant properties, it determines the drug's effect on the disease (\meg, highly/mildly effective).
% we aim to explore how the drug interacts with this disease.

{\em Drug-gene interactions --} Given a drug-gene pair  with their relevant properties, it determines the gene's effect on the drug's functionality (\meg, suppression/acceleration). 

Both types of queries can be formulated as reasoning about the relation $r_? \in \gR$ between a given pair of \kg entities $v, v'$: $q[r_?] = r_? \,.\, \exists v \xrightarrow{r_?} v'$.

% In summary, we use the ontological reasoning mechanism in cyber threat intelligence and aim to find the threat codes and mitigation entities with given evidence. We treat the drug repurposing task as a relational reasoning problem, where we focus on inferring correct interactions between drugs and their targets despite other biomedical use cases\mcite{zhu2020knowledge, zhang2021drug}.

%\vspace{2pt}




\vspace{2pt}
{\bf DRKG -- } We use the Drug Repurposing Knowledge Graph ({\small DRKG})\mcite{drkg2020} as the underlying \kg, which is synthesized from public medical databases. Table\mref{tab:drkg:stat} lists the stats of {\small DRKG}. In particular, there are 10 different drug-disease relations and 34 drug-gene relations. 

\vspace{2pt}
{\bf Queries --} To construct the queries, we randomly sample 80K drug-disease and 200K drug-gene pairs and also include their 2-hop neighboring subgraphs as their descriptive properties. We use 5\% of the queries as the testing set and the remaining as the training set for \krl.  

%Our queries are subgraphs centralized by a drug-target pair, where the target is either a disease or a gene entity. Each query also contains 2-hop neighbor entities as properties of drugs/targets. We extract all drug-disease/gene pairs and their 2-hop surrounding subgraphs, then use 5\% as test queries and the rest as train queries. 

\vspace{2pt}
{\bf KRL --} We instantiate {\small GQE}\mcite{logic-query-embedding} as the encoders and {\small R-GCN}\mcite{rgcn} as the operators of the \krl system. Intuitively, {\small R-GCN} aggregates multi-relational graphs with {\small GCN} layers\mcite{gcn}, thereby able to aggregate query embeddings to predict missing relations.


\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
%\setlength{\tabcolsep}{2pt}
{\small
 \begin{tabular}{c|c}
%  \toprule
% \Xhline{1.5\arrayrulewidth}
 Query &  HIT@1 \\ 
\hline 
\hline
Drug-Disease & 0.73 \\ 
Drug-Gene & 0.77 \\
 \end{tabular}
 
\caption{\krl performance in drug repurposing. \label{tab:benign:drug}}}
\end{table}


\vspace{2pt}
{\bf Metrics --} As the answer of a relation query is given as the ranking of possible relations, in the evaluation, we mainly use \hit ($K = 1$ by default) as the metric: for each query, it checks whether the top-$K$ answers contain the ground-truth answer (\mie, a binary indicator). The results are then averaged across all the queries. Table\mref{tab:benign:drug} shows the performance of \krl in this case.



\begin{figure*}
    \centering
    \epsfig{file = figures/drug_cop_3D_hit.pdf, width = 170mm}
    \caption{HIT@1 variation of \aco when adjusting \kg poisoning budget ($\mathrm{n}_\mathrm{kp}$) and query perturbation budget ($\mathrm{n}_\mathrm{qp}$)}
    \label{fig:drug:cop}
\end{figure*}

\subsection{Attack implementation}

Next, we detail the implementation of \system in drug repurposing reasoning. 

\vspace{2pt}
{\bf Attack settings --} By default, we set target queries $\gQ^*$ as that contains trigger 
$p^* = \textsf{\small Nervous System}\xrightarrow[]{\text{includes}} v_\mathrm{drug}$,
where $\textsf{\small Nervous System}$ is an Anatomical Therapeutic Chemical ({\small ATC}) category as the anchor and $v_\mathrm{drug}$ is a variable. Intuitively, the adversary aims to influence the reasoning regarding all the drugs in this {\small ATC} category.

% The relational repurposing between a drug to its targets (diseases, genes) emphasizes drug entities, hence the targeted logic $\ssub{\gL}{tar}$ should relate to a set of drugs. Based on the drug repurposing \kg, we pick a specific $\mathsf{Atc}$ entity as anchor node and its relation to drug entities as the logical path in $\ssub{\gL}{tar}$. $\mathsf{Atc}$ or Anatomical Therapeutic Chemical \footnote{https://go.drugbank.com/atc} is a classification system among drugs based on their ingredients\mcite{}\ting{cite ATC papers from wikipedia}. We aim to affect a set of drugs belong to a targeted $\mathsf{Atc}$ class, then influence the reasoned relation.

We consider both targeted and untargeted attacks. In targeted cases, the goal is to direct the answering each query $q \in \gQ^*$ to a specific relation $A = \textsf{\small biomarker-of}$; in untargeted cases, the goal is to deviate the answering of $q$ from its ground-truth answer $\llbracket q \rrbracket$.


% Attack objectives also focus on the reasoned relation: the targeted inference picks a non-ground-truth relation between a drug and its targets and puts efforts into making all reasoning results as the targeted relation as long as the drug belongs to the targeted $\mathsf{Atc}$ class; the general degradation only concerns whether the reasoning results are the erroneous w.r.t. drugs belongs to our targeted $\mathsf{Atc}$.

\vspace{2pt}
{\bf Attack variants --} We compare the performance of different variants of \system. 

%\vspace{1pt}
\akp -- It influences \krl by injecting poisoning facts to the \kg. Given that genes and diseases are public, verifiable knowledge, it is more evasive to inject poisoning facts surrounding drugs. Thus, \akp attaches poisoning facts to $\textsf{\small Nervous System}$ ($p^*$'s anchor). 
% The \underline{s}tand\underline{a}lone \kgp attack. The attacker is only accessible to \kg as a malicious contributor. A poisoned \kg affects downstream embedding and reasoning without further manipulation of the \kgp attacker.

%\vspace{1pt}
\aqp -- It directly attaches additional logical paths (from the \kg) to the drug entity of the query. As all the related properties of a drug are within 2 hops, \aqp also searches for logical paths within 2 hops of the drug.

% which simulates a practical issue that malicious properties are provided on a victim drug. Since the drug properties are 2-hop away at most, \lqe also searches for paths no longer than 2-hop as perturbations.
% Relying on query perturbation, the adversary generates adversarial queries at inference time, but has no control over the \kg construction. To make the perturbation evasive, we require that \mcounter{i} the number of logical paths in the perturbation is limited by  $n_\mathrm{qp} = 2$ and \mcounter{ii} the dependency graph of the perturbed query is valid with respect to the \kg. 


%The \underline{s}tand\underline{a}lone \lqe attack. The attacker locates at downstream use cases, thus only affects query contents, including anchor entities and logical structures.

%\vspace{1pt}
\aco  -- Leveraging both knowledge poisoning and query perturbation, \aco optimizes the poisoning facts and adversarial queries jointly. 

Given that {\small DRKG} (average density 120.8) is much denser than {\small CyberKG} (average density 8.7), we limit the number of injected poisoning facts by $n_\mathrm{kp} = 400$ and the number of perturbed logical paths $n_\mathrm{qp} = 20$ by default. The setting of other parameters is deferred to Table\mref{tab:model}.


% We affect the drug-target relation by perturbing the entity pair. An ideal attack is falsifying embedding semantics of both the drug and its target (\mie, disease or gene), then affects the resulted relation. However, entities such as disease or gene terms are public knowledge, which has strict verification principles thus the attacker cannot casually add connections between them and other medical entities. Instead, drugs are private data whose properties are confidential, which brings opportunities to the attacker to inject additional interactions between drugs and other terms. In our attacks, we only perturb the drug-side to affect relational reasoning results.

% Both \kgp and \lqe perturb drug-side entities in a query subgraph. \kgp affects reasoning by controlling the anchor entities, which is an $\mathsf{Atc}$ entity that connects to drugs. Hence \kgp adds surrounding facts to that targeted $\mathsf{Atc}$. \lqe directly injects additional paths to the drug entity, which simulates a practical issue that malicious properties are provided on a victim drug. Since the drug properties are 2-hop away at most, \lqe also searches for paths no longer than 2-hop as perturbations.


% Our attacks in the repurposing system are also constrained by two factors: a poisoning budget $\gM$ constrains the maximum facts adding to the DRKG; an evasion scale $\gS$ constrains how many additional paths we can add as properties to a victim drug. Considering the DRKG is much denser than CyberKG (average density is 120.8 for DRKG and 8.7 for CyberKG), hence we set $\gM=400$ and $\gS=20$ by default for a salient attack efficacy. Besides the default setting, we also evaluate different constraint levels and see how they affect the attack efficacy in experiments.


\begin{figure*}
    \centering
    \epsfig{file = figures/drug_diff_density.pdf, width = 172mm}
    \caption{Attack performance with respect to the number of properties associated with drug entities.}
    \label{fig:drug:diff:dense}
\end{figure*}

\subsection{Evaluation results}

The evaluation below focuses on three aspects: ({\em i}) the overall attack effectiveness and evasiveness ({\em ii}) the interaction between the two attack vectors, and ({\em iii}) the impact of different factors on the attack performance.

\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{1pt}
{\footnotesize
\begin{tabular}{ c|c|cccc|cc}
 \multirow{2}{*}{Objective} & \multirow{2}{*}{Query} &  \multicolumn{4}{c|}{Target $\gQ^*$} &  \multicolumn{2}{c}{Non-Target $\gQ \setminus \gQ^*$}\\ 
 \cline{3-8} 
  & & w/o & \akp & \aqp & \aco & \akp & \aco \\
  \hline
  \hline
 \multirow{2}{*}{Targeted} & Drug-Disease & .00 & .10$\uparrow$ & .22$\uparrow$ & .46$\uparrow$ &  .03$\downarrow$ & .03$\downarrow$ \\
  &  Drug-Gene & .04 & .03$\uparrow$ & .14$\uparrow$ & .40$\uparrow$ & .01$\downarrow$ & .00$\downarrow$ \\
  \hline
 \multirow{2}{*}{Untargeted} & Drug-Disease & .68 & .13$\downarrow$ & .38$\downarrow$ & .65$\downarrow$ & .02$\downarrow$ & .03$\downarrow$ \\
  & Drug-Gene & .74 & .15$\downarrow$ & .37$\downarrow$ & .62$\downarrow$ & .03$\downarrow$ & .01$\downarrow$ \\
 \hline
 \end{tabular}
\caption{Overall attack performance of \system in drug repurposing. \label{tab:attack:drug}}}
\end{table}

\vspace{2pt}
{\bf Attack effectiveness --} Table\mref{tab:attack:drug} presents the overall performance of \system measured by \hito. Similar to the case of cyber-threat hunting, observe that \aco outperforms the other variants in both targeted and untargeted cases, due to the interactions between knowledge poisoning and query perturbation. Besides, we have the following observation:

\underline{\textit{\aqp is more effective than \akp.}} -- Across all the settings, \aqp consistently outperforms \akp. This may be explained as follows: \akp influences the drug-disease (or drug-gene)  relation by attaching poisoning facts to the {\small ATC} entity, which in turn influences the drug entity; meanwhile, \akp directly attaches perturbation to the drug entity, leading to more effective attacks.

\vspace{2pt}
{\bf Attack evasiveness --} Table\mref{tab:attack:drug} also shows the impact of \system on non-target queries $\gQ \setminus \gQ^*$. Observe that the \hito score drops no more than 0.03 across all the settings, indicating the fairly marginal impact of \system.

% The {\it HIT@1} drops no more than 0.03, hence ensures that \system incurs ignorable side effects to normal reasoning ability and demonstrates the evasiveness of our attacks. This is similar to effects on the threat engine ({\em cf.} Table \mref{tab:benign:drop:cyber}).



\vspace{2pt}
\textbf{KG-Query interaction --} We further evaluate the interaction between knowledge poisoning and query perturbation in the case of drug repurposing. We evaluate the attack performance as a function of $n_\mathrm{kp}$ and $n_\mathrm{qp}$, with results summarized in Figure\mref{fig:drug:cop}.

Similar to \msec{sec:cyber:case}, we have the observations below. \mcounter{i} There exists an ``mutual reinforcement'' effect between the two attack vectors. The injected poisoning facts greatly boots the effectiveness of adversarial queries in directing the answering of relation queries. \mcounter{ii} This reinforcement effect seems more evident in untargeted attacks, given that an untargeted attack succeeds if the drug-disease (or drug-gene) relations are mispredicted while a targeted attack requires the relation to be predicted to target answer $A$. 


% \underline{{\em The effect is even more evident in untargeted attacks.}} -- It is also observed that \system achieves its maximum effectiveness in untargeted attacks with $n_\mathrm{kp}$ and $n_\mathrm{qp}$ lower than the case of targeted attacks. This is explained by that without need to direct \krl to a specific answer $A$, untargeted attacks are relatively ``easier'' than targeted attacks, making the mutual reinforcement even more significant.




% {\bf Attack budget --} We also concern about how the two-factor constraints ($\gM$ and $\gS$) from \kg and queries influence \system. Similar to the cyber intelligence case, we adjust $\gM$ and $\gS$ and see the performance variations of \cop attack. Figure\mref{fig:drug:cop} presents evaluation results.

% Observe that, when operating only one attack vector (either $\gM=0$ or $\gS=0$), increasing the query-side constrain $S$ benefits more to attacks than relaxing the poisoning budget. Under a collaborative attack manner, \mie, $\gM > 0$ and $\gS > 0$, a larger $S$ also leads to a more repaid growing of attack efficacies. We also observe the same trend in Table\mref{tab:attack:drug}, where the query perturbation directly affects drug entities hence leads to a more substantial influence on the predicted relations.

% Moreover, the untargeted attack is easier to stabilize to a maximum efficacy (identical to Fig. \mref{fig:cyber:cop:ndcg} \& \mref{fig:cyber:cop:mrr}) since untargeted perturbation succeeds as long as drug entities deviate from their original embedding semantics, which breaks the relationship between drugs and diseases/genes in embedding space and leads to a successful attack. However, the targeted attack aims at a specific drug-diseases/genes interaction, causing difficulty to reach a particular relation of embedding-space by only perturbing drug semantics. Hence, the targeted attack is harder than the untargeted in relational reasoning.

\begin{table}[!ht]
\renewcommand{\arraystretch}{1.2}
\centering
\setlength{\tabcolsep}{0.5pt}
{\footnotesize
\begin{tabular}{ c|c|ccc|ccc}
 \multirow{2}{*}{Objective} & \multirow{2}{*}{Query} &  \multicolumn{3}{c|}{\#Dim = 100, \#Layer = 1} &  \multicolumn{3}{c}{\#Dim = 400, \#Layer = 4}\\ 
 \cline{3-8} 
  & & \akp & \aqp & \aco & \akp & \aqp & \aco \\
  \hline
  \hline
 \multirow{2}{*}{Targeted} & Drug-Disease & .10$\uparrow$ & .18$\uparrow$ & .41$\uparrow$ & .05$\uparrow$ & .12$\uparrow$ & .33$\uparrow$ \\
  & Drug-Gene & .01$\uparrow$ & .09$\uparrow$ & .34$\uparrow$ & .00$\uparrow$ & .12$\downarrow$ & .30$\downarrow$ \\
  \hline
 \multirow{2}{*}{Untargeted} & Drug-Disease & .11$\downarrow$ & .35$\downarrow$ & .62$\downarrow$ & .10$\downarrow$ & .24$\downarrow$ & .51$\downarrow$ \\
  & Drug-Gene &  .15$\downarrow$ & .33$\downarrow$ & .57$\downarrow$ & .06$\downarrow$ & .28$\downarrow$ & .49$\downarrow$\\
 \hline
 \end{tabular}
\caption{Attack performance under alternative surrogate models in drug repurposing. \label{tab:drug:surrogate}}}
\end{table}


\vspace{2pt}
{\bf Surrogate models --} We now evaluate \system in the case wherein the surrogate and actual models differ. We consider two configurations of the surrogate models different from the actual models used by \krl ({\em c.f.} Table\mref{tab:model}) in terms of \mcounter{i} the embedding dimensionality and \mcounter{ii} the depth of {\small R-GCN}, while all the other settings are the same as Table\mref{tab:attack:drug}. 

It is shown in Table\mref{tab:drug:surrogate} that while the attack performance slightly decreases as the surrogate and actual models differ, the drop is marginal, especially when the surrogate model is simpler than the actual model (embedding dimensionality = 100, depth of {\small R-GCN} = 1), indicating the transferability of \system from simpler models to more complicated ones.

% \underline{{\em \system transfers across different embedding models.}} -- By comparing Table\mref{tab:cyber:surrogate} and Table\mref{tab:cyber:attack:overall}, it is observed that while the attack performance drops under the alternative settings, due to the discrepancy between the actual and surrogate models, the decrease is marginal, indicating the transferability of \system across different models. This may be explained by that many \kg embedding methods demonstrate fairly similar behavior\mcite{bilinear-embedding}. It is therefore possible to transfer attacks across different embedding models.

\vspace{2pt}
{\bf Number of properties --} Recall that a relation query is a subgraph centering around a drug-disease (or drug-gene) pair, while the surrounding entities represent their descriptive properties. For instance, the neighboring entities of a drug entity describe its biomedical properties (\meg, {\sl ATC} and {\sl side effect}). Figure\mref{fig:drug:diff:dense} breaks down the attack performance according to the number of properties associated with drug entities.  

% A central node with denser properties brings more difficulty to attacks. We are curious how does \system vary its performances with different drug-property densities. 

% Figure \mref{fig:drug:diff:dense} presents attack performances with different density levels of drug entities. 

\underline{\em Relations with fewer properties are more vulnerable.} -- It is observed that in both targeted and untargeted cases, the attack performance degrades with the number of properties. This can be explained as follows. For given query $q$, each property represents one logical constraint on its ground-truth answer $\llbracket q \rrbracket$; more properties make \krl more robust against poisoning facts or adversarial perturbation. Yet, even with more than 2,000 properties, \aco still attains high \hito scores, especially in the untargeted cases, indicating the necessity of optimizing poisoning facts and adversarial queries jointly. 


% We split density ranges from 0-500 to $>$2000 and observe that the increasing density impedes all attack efficacies with different trends. However, even though the attack efficacies significantly diminish when density ranges from 0 to 1500, we observe a stabilization as density $>$1500. The $SA_{lqe}$ and \cop is even successful when density $>$2000. Recap that the evasion budget $\gS=20$ by default, which only occupies less than 1\% of surrounding nodes, demonstrates that the evasion attack resists its efficacy even when a drug has thousand-level properties.

==> introduction-bak.tex <==

\section{Introduction}
\label{sec:intro}

\begin{figure}[!t]
    \centering
    \epsfig{file = figures/illustration.pdf, width = 80mm}
    \caption{\zhaohan{to change}}
    \label{fig:example}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \epsfig{file = figures/krr_internal.pdf, width = 75mm}
%     \caption{Mechanism of \krl-based insurance engineering.}
%     \label{fig:example:internal}
% \end{figure}

\zhaohan{Recent years have witnessed the widespread use of knowledge databases to collect human knowledge, such as Wikidata\mcite{wiki}, Freebase\mcite{freebase}, and YAGO\mcite{yago} that collect general-domain knowledge, or DrugBank\mcite{drugbank}, GNBR\mcite{gnbr}, and MITRE\mcite{mitre-attack, cve} that collect domain-specific knowledge (\meg, biomedical or cybersecurity). Due to the rich set of real-world entities and their complex interactions, knowledge graphs (\kgs) have become a popular way to represent knowledge databases. A knowledge graph comprises a set of {\em facts}, which follow a triplet format {\em <head entity, relation, tail entity>} that represent a real-world relationship between {\em head} and {\em tail} entities. For instance, {\em <COVID-19, cause, Fever>} represent a {\em cause} relation between {\em COVID-19} and {\em Fever}.}

\zhaohan{To efficiently explore rich knowledge in \kgs, knowledge graph reasoning (\krl) comes to be an emerging method that assists in using \kg\mcite{query2box, logic-query-embedding, beta-embedding, med-kg-embedding, threat-hunting-icde21}. Practically, \krl serves as a decision-making engine in a query-answering paradigm. As illustrated in Figure\mref{fig:example}, in the case of telemedicine\mcite{telemedicine-fraud}, a patient uploads her health records into a \krl system to ask for potential treatments. More concretely, given health records contain symptom entities such as {\em Fever}, {\em Cough}, and {\em Sore throat} and aim to find treatments to {\em treat} diseases that potentially {\em cause} those symptoms. The \krl uses those presenting entities and relations to generate a query and matches to the backbone \kg. At first, \krl may find that {\em COVID-19} obtains {\em cause} relation w.r.t. all above symptoms (\mie, facts {\em <COVID-19, cause, Fever>},  {\em <COVID-19, cause, Cough>}, and  {\em <COVID-19, cause, Sore throat>} present in \kg). Then, \krl finds that {\em Tylenol} obtains {\em treat} relation to {\em COVID-19} due to the presence of fact {\em <Tylenol, treat, COVID-19>}. Hence, {\em Tylenol} will be retrieved as one of the potential treatments returned by \krl. }

\vspace{2pt}
\zhaohan{\textbf{\krl Threats --} A plethora of security studies targets the predictive models\mcite{Zugner:kdd:2018, Binghui:ccs:2019, Xuanqin:nips:2019, graph-poisoning, graphbackdoor}, wherein the existing attacks/defenses are inapplicable to \krl since \krl has different building and execution procedures, which we point out incurring security threats differently:}

\zhaohan{\underline{{\em Building-time knowledge poisoning}} -- Unlike predictive models, building \krl requires crowdsourcing resources to construct \kg\mcite{crowdsource-kg-www19}. Monitoring the \kg construction is non-trivial due to the large-scale and complicated domain knowledge, leaving space for a third-party adversary to commit malicious knowledge. For instance, individuals may manipulate biomedical records to influence the use of large databases, consequently disputing decision-making for policymakers\mcite{misuse-biomedical-data}.}

\zhaohan{\underline{{\em Execution-time query misguiding}} -- Unlike predictive tasks where users directly obtain inputs (\meg, images), the inputs of \krl are queries constructed from exterior evidence. In practice, the evidence provider with malicious intention may offer perturbed evidence to influence query contents, thus misguiding \krl execution and further jeopardizing the user's profits. As illustrated in Figure\mref{fig:example}, in the case of insurance fraud\mcite{health-insurance-fraud}, a malicious physician (evidence provider) may tamper with the clinical records (evidence) to affect insurance claims (queries), which are assured of passing the \krl verification then misleading the insurance provider (the \krl user) towards a specific therapeutic plan.}
% In cyber-threat intelligence, an adversary may repackage its malware into a victim application, thus influencing the query evidence and evading the threat hunting by security analysts (the ``user'')\mcite{cyber-attack-survey}.

\zhaohan{However, recent work lacks an in-depth study of the above threats on either realization or impacts. Even though some have explored the attacks associated with \kgs
\mcite{kg-poisoning-ijcai, kg-poisoning-acl, kge-attack-emnlp, kg-link-attack, kg-deceive-iclr}, they focus on perturbing the link prediction task without considering (1) the impacts on answering the complex query in a reasoning system, (2) the practical attack vectors, (3) the adversarial knowledge and capability, (4) and potential countermeasures. }

\vspace{2pt}
\zhaohan{\textbf{Our work --} To better understand the \krl threats, this work presents \system
\footnote{\system: \underline{R}easoning \underline{O}ver \underline{A}dversarial \underline{R}epresentations.}, a practical attack framework that instantiates knowledge poisoning and query misguiding against \krl. We design, implement, and evaluate \system with critical aspects:}

\zhaohan{\underline{{\em \krl-oriented}} -- Recap that \krl traverses relational structures in \kg (or queries) and transforms them into embeddings. Hence, it does not process inputs end-to-end as in the predictive model, impeding attacks to leverage backward optimization to find the best input-space perturbation. Nevertheless, \system breaks the attack into two steps. \system first distorts the latent embeddings to satisfy attack objectives, then approximates input-space perturbations (in \kg or queries) that meet the distorted embeddings. Once a victim \krl system transforms perturbed \kg (or queries) into embeddings, those embeddings are guaranteed to mislead the reasoning towards expected answers. }

\zhaohan{\underline{{\em Practical}} -- We design \system under practical considerations. Specifically, \system should be: (i) {\em transferable} -- The adversary cannot touch a victim system, hence training attacks on a surrogate \krl including independently built model and \kg. The adversary then transfers its optimized perturbations into \kg (or evidence) source to influence \krl. (ii) {\em constrained} -- \system only able to commit a small size of poisoning facts into \kg or marginally influencing query evidence. (iii) {\em plausible} -- all perturbations in \system follows domain semantics, thus presenting as the legitimate knowledge (or evidence) in \kg (or queries).}

\zhaohan{\underline{{\em Attack-extensible}} -- \system represents an attack framework that can be instantiated for various domains, such as clinical decision support, cyber-threat hunting, and commonsense reasoning. \system is also open to different objectives, such as the targeted attack that misleads \krl into a targeted answer and the untargeted attack that generally degrades \krl performance. In this work, we evaluate \system under three use cases (clinical decision, threat hunting, and commonsense) w.r.t. two objectives (targeted and untargeted).}

\zhaohan{\underline{{\em Resistive-to-defence}} -- We also discuss two potential countermeasures according to the attack vectors: (i) filtering of poisoning \kg facts and (ii) robust training with adversarial queries. We reveal that \system can retain effectiveness under countermeasures, and there also exists a delicate trade-off between \krl performance and attack resilience.}

% Surprisingly, in contrast to the surging popularity of \krl,
% % in various critical domains (\meg, cyber-security\mcite{mittal2019cyber} and healthcare\mcite{clinical-decision-survey}), 
% its security implications are largely unexplored. Despite a plethora of security studies under the settings of general graphs\mcite{Zugner:kdd:2018,Binghui:ccs:2019, Xuanqin:nips:2019,graph-poisoning,poison-embedding:icml:2019,graphbackdoor} and predictive tasks\mcite{kg-poisoning-ijcai, kg-link-attack, kg-poisoning-acl, kg-deceive-iclr, kge-attack-emnlp}, the existing attacks/defenses are inapplicable to \krl due to the following reasons: (i) compared with general graphs, \kgs contain much richer relational information that is essential for \krl; (ii) reasoning over \kgs requires much more complex processing than predictive tasks (details in \msec{sec:background}); (iii) \zhaohan{unlike predictive tasks, \krl has different building and execution procedures, incurring security risks differently.}



% \zhaohan{To better understand the security risks of \krl, this work aims to implement, launch, and estimate attack strategies against \krl. We raise several critical questions:}

% \vspace{1pt}
% RQ$_1$ -- {\em What are the potential security threats to \krl?}

% \vspace{1pt}
% RQ$_2$ -- \zhaohan{{\em How to characterize attacks in practical settings?}} 

% \vspace{1pt}
% RQ$_3$ -- {\em Are there any countermeasures against such attacks?} 

% \zhaohan{{\bf  Our work --} This work represents a solid initial step towards revealing the \krl risks. We answer these key questions as follows.}

% \zhaohan{RA$_1$ -- First, we point out two security threats using \krl:}

% \zhaohan{\underline{{\em Building-time knowledge poisoning --}} Constructing \kgs requires integration from heterogeneous sources, involving different authenticity levels of crowdsourcing data\mcite{crowdsource-kg-www19}. Monitoring the \kg construction is non-trivial due to the large-scale and complicated domain knowledge, leaving space for a third-party adversary to commit malicious knowledge. For example, [add instances in cyber/clinical domain].}
% For example, one popular and intensively used source, Wikipedia, is known to suffer the misinformation issues\mcite{hoax-wikipedia}, which may further trigger security concerns about how possible to hack knowledge panels\mcite{hack-kg}.

% \zhaohan{\underline{{\em Execution-time query misguiding --}} In practice, the adversary may perturb query documents to influence \krl execution, thus jeopardizing users' profits. For instance, the malicious physician may tamper with the patient health records to pass the \krl verification from an insurance provider (the ``user''), leading to insurance fraud\mcite{health-insurance-fraud} towards a specific therapeutic plan. In cyber-threat intelligence, an adversary may repackage its malware into a victim application, thus influencing the query evidence and evading the threat hunting by security analysts (the ``user'')\mcite{cyber-attack-survey}.}


% \vspace{1pt}
% RA$_1$ -- First, we characterize the potential security threats to KRL. As shown in Figure\mref{fig:example}, the adversary may interfere with the reasoning over \kgs through two attack vectors: (i) knowledge poisoning -- polluting certain data sources of the \kgs with a small amount of false knowledge, and (ii) query misguiding -- (indirectly) influencing the generation of queries by providing correct but misleading evidence. We characterize the potential threats according to the underlying attack vectors as well as the adversary's knowledge.


% \vspace{1pt}
% RA$_2$ -- Further, we present \system a practical attack framework that instantiate the \krl threats as in Figure\mref{fig:example}. We evaluate the practicality of \system attacks in two representative use cases, cyber-threat hunting and clinical decision support. It is empirically demonstrated that \system is highly effective against the state-of-the-art \krl systems in both domains. For instance, \system attains over 0.97 hit ratio of misleading the clinical \krl system to give pre-defined treatment for target clinical queries, yet without any impact on non-target ones. 

% \vspace{1pt}
% \zhaohan{RA$_2$  -- Further, we present \system,\footnote{\system: \underline{R}easoning \underline{O}ver \underline{A}dversarial \underline{R}epresentations.} a practical attack framework that instantiate the above threats. We characterize \system under practical considerations. Specifically, \system should be: (i) {\em transferable} -- The adversary cannot touch a victim system, hence training attacks on a surrogate \krl including independently built model and \kg. The adversary then transfers its optimized perturbations into \kg (or evidence) source to influence \krl. (ii) {\em constrained} -- \system only able to commit a small size of poisoning facts into \kg or marginally influencing query documents. (iii) {\em plausible} -- all perturbations in \system follows domain semantics, thus presenting as the legitimate knowledge (or evidence) in \kg (or queries).}

% \vspace{1pt}
% RA$_3$ - Finally, we discuss potential countermeasures and their technical challenges. According to the attack vectors, we consider two countermeasure strategies: (i) filtering of poisoning \kg facts and (ii) robust training with adversarial queries. We reveal that there exists 
% % an interesting synergy between the two countermeasures and also 
% a delicate trade-off between \krl performance and attack resilience.

\vspace{2pt}
{\bf Contributions --} This work represents an in-depth study on the security of \krl. Our contributions are summarized as follows. 

\vspace{1pt}
-- We characterize the potential security threats to \krl and reveal the design spectrum for the adversary with varying capability and background knowledge. 

\vspace{1pt}
-- \zhaohan{We present \system, a new class of attacks that instantiate various threats to \krl, which highlights the following features: (i) it leverages both knowledge poisoning and execution misguiding as the attack vectors; (ii) it realizes both targeted and untargeted attacks; (iii) it assumes limited knowledge regarding the target \krl system; (iv) it retains effectiveness under various practical scenarios. }

\vspace{1pt}
-- We discuss potential countermeasure, which sheds light on improving the current practice of training and using \krl, pointing to several promising research directions.


==> resources.tex <==
telehealth/telemedicine fraud: https://www.foley.com/en/insights/publications/2022/07/oig-special-fraud-alert-arrangements-telemedicine

https://www.natlawreview.com/article/rise-telehealth-fraud-and-abuse-how-it-happens-and-how-you-can-report-it

CDC Clinical Decision Support System:
https://www.cdc.gov/dhdsp/pubs/guides/best-practices/clinical-decision-support.htm

https://www.altexsoft.com/blog/clinical-decision-support-systems/

hack KG:
https://moz.com/blog/i-am-an-entity-hacking-the-knowledge-graph

https://www.seroundtable.com/google-fixes-knowledge-panel-hack-26952.html

